Should We Adjust for the Test for Pre-trends in Difference-in-Difference Designs?

The common practice in difference-in-difference (DiD) designs is to check for parallel trends prior to treatment assignment, yet typical estimation and inference does not account for the fact that this test has occurred. I analyze the properties of the traditional DiD estimator conditional on having passed (i.e. not rejected) the test for parallel pre-trends. When the DiD design is valid and the test for pre-trends confirms it, the typical DiD estimator is unbiased, but traditional standard errors are overly conservative. Additionally, there exists an alternative unbiased estimator that is more efficient than the traditional DiD estimator under parallel trends. However, when in population there is a non-zero pre-trend but we fail to reject the hypothesis of parallel pre-trends, the DiD estimator is generally biased relative to the population DiD coefficient. Moreover, if the trend is monotone, then under reasonable assumptions the bias from conditioning exacerbates the bias relative to the true treatment effect. I propose new estimation and inference procedures that account for the test for parallel trends, and compare their performance to that of the traditional estimator in a Monte Carlo simulation.

==> Figures/WorkAdvanceSimulation/CumulativeBiasWide_0rows.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Mon Apr 30 10:51:07 2018
 0 & Unconditional & 100 & 4152 & 0 & 0 \\ 
  0 & Conditional & 80 & 4152 & 0 & 0 \\ 
  


==> Preambles/header_beamer.tex <==
% Typesetting
	\usepackage{amsfonts}
	\usepackage{amssymb}

	\usepackage{subfig}

	\usepackage{graphicx}
    
    \usepackage{tikz}
    \usetikzlibrary{positioning}
    \usetikzlibrary{snakes}
    \usetikzlibrary{calc}
    \usetikzlibrary{arrows}
    \usetikzlibrary{decorations.markings}
    \usetikzlibrary{shapes.misc}
    \usetikzlibrary{matrix,shapes,arrows,fit,tikzmark}
    
    %%% TIKZ STUFF
    \tikzset{   
            every picture/.style={remember picture,baseline},
            every node/.style={anchor=base,align=center,outer sep=1.5pt},
            every path/.style={thick},
            }
    \newcommand\marktopleft[1]{%
        \tikz[overlay,remember picture] 
            \node (marker-#1-a) at (-.3em,.3em) {};%
    }
    \newcommand\markbottomright[1]{%
        \tikz[overlay,remember picture, baseline=-.1pt] 
            \node (marker-#1-b) at (0em,0em) {};%
    }
    \tikzstyle{every picture}+=[remember picture] 
    \tikzstyle{mybox} =[draw=black, very thick, rectangle, inner sep=10pt, inner ysep=20pt]
    \tikzstyle{fancytitle} =[draw=black,fill=red, text=white]
    %%%% END TIKZ STUFF
    
    \usepackage{color}
    \definecolor{LightCyan}{rgb}{0.88,1,1}

% Bibliography
    % \usepackage[style=authoryear-comp,natbib=true,backend=biber]{biblatex}
    % \addbibresource{Bibliography.bib}
    % \usepackage{csquotes}
	\usepackage{natbib}
 	\bibliographystyle{apalike}
	
	\usepackage{bibunits}
	\defaultbibliography{Bibliography.bib}  
	\defaultbibliographystyle{apalike}

	
% Links
	\usepackage{hyperref}
	\hypersetup{
    colorlinks=true,
    linkcolor=black,
    filecolor=magenta,      
    urlcolor=blue,
    citecolor = black
}
	\usepackage{cleveref}

% Todonotes
	\usepackage[framemethod=tikz]{mdframed}
	\usepackage{todonotes}
	\presetkeys{todonotes}{color=black!5,inline}{} % noline

% Boxes
    \usepackage{tcolorbox}
    \newtcbox{\feedback}{nobeforeafter,colframe=black,colback=white,boxrule=0.5pt,arc=2pt,
      boxsep=0pt,left=2pt,right=2pt,top=2pt,bottom=2pt,tcbox raise base}
      
% Theorems
    \usepackage{amsthm}
     
    \newtheorem{thm}{Theorem}
    \newtheorem{asm}{Assumption}
    \newtheorem{con}{Conjecture}
    \newtheorem{prop}{Proposition}
    \newtheorem{lem}{Lemma}
    \newtheorem{cor}{Corollary}
    \newtheorem{rem}{Remark}
    \newtheorem{defn}{Definition}

%Packages and commands for column widths in tables
\usepackage{array}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

%Turn off toolbar
\setbeamertemplate{navigation symbols}[default]
\beamertemplatenavigationsymbolsempty  


==> Tables/WorkAdvanceSimulation/CumulativeBias.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Sun Apr 29 19:32:39 2018
 cumulativeTreatmentEffect & 4152 & 5972 & 6331 & 7792 & 8625 & 9612 & 11023 & 11432 & 13308 \\ 
  cumulativeBias & 0 & 1820 & 2179 & 3640 & 4474 & 5460 & 6872 & 7280 & 9157 \\ 
  percentBias & 0 & 44 & 52 & 88 & 108 & 132 & 166 & 175 & 221 \\ 
  \onslide<2->{acceptPretrends} & 100 & 100 & 66 & 100 & 34 & 100 & 9 & 100 & 1 \\ 
  


==> Tables/WorkAdvanceSimulation/CumulativeBiasWide.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Sun Apr 29 21:02:34 2018
 0 & Unconditional & 100 & 4152 & 0 & 0 \\ 
  0 & Conditional & 80 & 4152 & 0 & 0 \\ 
  20 & Unconditional & 100 & 5972 & 1820 & 44 \\ 
  20 & Conditional & 66 & 6331 & 2179 & 52 \\ 
  40 & Unconditional & 100 & 7792 & 3640 & 88 \\ 
  40 & Conditional & 34 & 8625 & 4474 & 108 \\ 
  60 & Unconditional & 100 & 9612 & 5460 & 132 \\ 
  60 & Conditional & 9 & 11023 & 6872 & 166 \\ 
  80 & Unconditional & 100 & 11432 & 7280 & 175 \\ 
  80 & Conditional & 1 & 13308 & 9157 & 221 \\ 
  


==> Tables/WorkAdvanceSimulation/CumulativeBiasWide_0.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Mon Apr 30 11:58:14 2018
 0 & Unconditional & 100 & 4152 & 0 & 0 \\ 
  0 & Conditional & 80 & 4152 & 0 & 0   


==> Tables/WorkAdvanceSimulation/CumulativeBiasWide_0rows.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Mon Apr 30 10:51:07 2018
 0 & Unconditional & 100 & 4152 & 0 & 0 \\ 
  0 & Conditional & 80 & 4152 & 0 & 0 \\ 
  


==> Tables/WorkAdvanceSimulation/CumulativeBiasWide_20.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Mon Apr 30 11:58:14 2018
 20 & Unconditional & 100 & 5972 & 1820 & 44 \\ 
  20 & Conditional & 66 & 6331 & 2179 & 52   


==> Tables/WorkAdvanceSimulation/CumulativeBiasWide_40.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Mon Apr 30 11:58:14 2018
 40 & Unconditional & 100 & 7792 & 3640 & 88 \\ 
  40 & Conditional & 34 & 8625 & 4474 & 108   


==> Tables/WorkAdvanceSimulation/CumulativeBiasWide_60.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Mon Apr 30 11:58:14 2018
 60 & Unconditional & 100 & 9612 & 5460 & 132 \\ 
  60 & Conditional & 9 & 11023 & 6872 & 166   


==> Tables/WorkAdvanceSimulation/CumulativeBiasWide_80.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Mon Apr 30 11:58:14 2018
 80 & Unconditional & 100 & 11432 & 7280 & 175 \\ 
  80 & Conditional & 1 & 13308 & 9157 & 221   


==> Tables/WorkAdvanceSimulation/CumulativeBias_0.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Sun Apr 29 20:47:02 2018
 Treatment Effect & 4152 & 4152 \\ 
  Bias & 0 & 0 \\ 
  Bias (\%) & 0 & 0 \\ 
  Accept Pretrends (\%) & 100 & 80 \\ 
  


==> Tables/WorkAdvanceSimulation/CumulativeBias_20.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Sun Apr 29 20:47:02 2018
 Treatment Effect & 5972 & 6331 \\ 
  Bias & 1820 & 2179 \\ 
  Bias (\%) & 44 & 52 \\ 
  Accept Pretrends (\%) & 100 & 66 \\ 
  


==> Tables/WorkAdvanceSimulation/CumulativeBias_40.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Sun Apr 29 20:47:02 2018
 Treatment Effect & 7792 & 8625 \\ 
  Bias & 3640 & 4474 \\ 
  Bias (\%) & 88 & 108 \\ 
  Accept Pretrends (\%) & 100 & 34 \\ 
  


==> Tables/WorkAdvanceSimulation/CumulativeBias_60.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Sun Apr 29 20:47:02 2018
 Treatment Effect & 9612 & 11023 \\ 
  Bias & 5460 & 6872 \\ 
  Bias (\%) & 132 & 166 \\ 
  Accept Pretrends (\%) & 100 & 9 \\ 
  


==> Tables/WorkAdvanceSimulation/CumulativeBias_80.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Sun Apr 29 20:47:03 2018
 Treatment Effect & 11432 & 13308 \\ 
  Bias & 7280 & 9157 \\ 
  Bias (\%) & 175 & 221 \\ 
  Accept Pretrends (\%) & 100 & 1 \\ 
  


==> Tables/WorkAdvanceSimulation/SEsAndCoverage.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Tue Apr 17 21:16:24 2018
   0 & 0.97 & 0.93 & 1.00 & 0.04 & 0.05 \\ 
    1 & 0.97 & 0.92 & 1.00 & 0.04 & 0.05 \\ 
    2 & 0.97 & 0.93 & 1.00 & 0.04 & 0.05 \\ 
    3 & 0.97 & 0.93 & 1.00 & 0.04 & 0.05 \\ 
    4 & 0.96 & 0.91 & 1.00 & 0.04 & 0.05 \\ 
    5 & 0.96 & 0.91 & 1.00 & 0.04 & 0.05 \\ 
    6 & 0.96 & 0.91 & 1.00 & 0.04 & 0.05 \\ 
    7 & 0.96 & 0.91 & 1.00 & 0.04 & 0.05 \\ 
    8 & 0.96 & 0.92 & 1.00 & 0.04 & 0.05 \\ 
    9 & 0.97 & 0.92 & 1.00 & 0.04 & 0.05 \\ 
   10 & 0.97 & 0.92 & 1.00 & 0.04 & 0.05 \\ 
   11 & 0.96 & 0.92 & 1.00 & 0.04 & 0.05 \\ 
   12 & 0.97 & 0.94 & 1.00 & 0.04 & 0.05 \\ 
  


==> scrap.tex <==
\begin{frame}{FORMAT ME}


%\caption{Mean Estimate of Treatment Effect on Total Earnings, By Specification}
\setlength{\extrarowheight}{5pt}

\resizebox{.9\linewidth}{!}{  
\begin{tabular}{R{.15 \columnwidth} R{.2 \columnwidth} R{.15 \columnwidth} R{.15 \columnwidth} R{.1 \columnwidth} R{.1 \columnwidth} } 
Underlying Slope & Conditional & Accept Pretrends (\%) & Treatment Effect & Bias & Bias (\%) \\ \hline
 \input{Tables/WorkAdvanceSimulation/CumulativeBiasWide_0.tex}\\
 
 \marktopleft{a1} \onslide<2->{ \input{Tables/WorkAdvanceSimulation/CumulativeBiasWide_20.tex} } \markbottomright{a1}{red} \\
 
 \onslide<3->{\marktopleft{b1} \input{Tables/WorkAdvanceSimulation/CumulativeBiasWide_40.tex} \markbottomright{b1}{red}} \\

  \onslide<4->{\input{Tables/WorkAdvanceSimulation/CumulativeBiasWide_60.tex}} \\
 
\end{tabular}
}    

\uncover<2>{\tikz[overlay,remember picture,inner sep=1pt]
\node[draw=red,rounded corners,fit=(marker-a1-a.north west) (marker-a1-b.south east)] {};}

 \uncover<3>{\tikz[overlay,remember picture,inner sep=1pt]
 \node[draw=red,rounded corners,fit=(marker-b1-a.north west) (marker-b1-b.south east)] {};}
\end{frame}


%%%%%%%%%%%%%

\begin{frame}{FORMAT ME}


%\caption{Mean Estimate of Treatment Effect on Total Earnings, By Specification}
\setlength{\extrarowheight}{5pt}

%\resizebox{.9\linewidth}{!}{  
\begin{tabular}{R{.15 \columnwidth} R{.2 \columnwidth} R{.15 \columnwidth} R{.15 \columnwidth} R{.1 \columnwidth} R{.1 \columnwidth} } 
Underlying Slope & Conditional & Accept Pretrends (\%) & Treatment Effect & Bias & Bias (\%) \\ \hline
 \input{Tables/WorkAdvanceSimulation/CumulativeBiasWide_0.tex}\\
 
 \marktopleft{a1} \input{Tables/WorkAdvanceSimulation/CumulativeBiasWide_20.tex}  \markbottomright{a1}{red} \\
 
 \marktopleft{b1} \input{Tables/WorkAdvanceSimulation/CumulativeBiasWide_40.tex} \markbottomright{b1}{red} \\

  \input{Tables/WorkAdvanceSimulation/CumulativeBiasWide_60.tex} \\
 
\end{tabular}
%}    

\uncover<2>{\tikz[overlay,remember picture,inner sep=1pt]
\node[draw=red,rounded corners,fit=(marker-a1-a.north west) (marker-a1-b.south east)] {};}

 \uncover<3>{\tikz[overlay,remember picture,inner sep=1pt]
 \node[draw=red,rounded corners,fit=(marker-b1-a.north west) (marker-b1-b.south east)] {};}
\end{frame}

